The MultiBERTs: BERT Reproductions for Robustness Analysis

Experiments with pre-trained models such as BERT are often based on a single checkpoint. While the conclusions drawn apply to the artifact tested in the experiment (i.e., the particular instance of the model), it is not always clear whether they hold for the more general procedure which includes the architecture, training data, initialization scheme, and loss function. Recent work has shown that repeating the pre-training process can lead to substantially different performance, suggesting that an alternate strategy is needed to make principled statements about procedures. To enable researchers to draw more robust conclusions, we introduce the MultiBERTs, a set of 25 BERT-Base checkpoints, trained with similar hyper-parameters as the original BERT model but differing in random weight initialization and shuffling of training data. We also define the Multi-Bootstrap, a non-parametric bootstrap method for statistical inference designed for settings where there are multiple pre-trained models and limited test data. To illustrate our approach, we present a case study of gender bias in coreference resolution, in which the Multi-Bootstrap lets us measure effects that may not be detected with a single checkpoint. We release our models and statistical library along with an additional set of 140 intermediate checkpoints captured during pre-training to facilitate research on learning dynamics.

==> unused/experimental-old.tex <==
\section{Application of Multi-Bootstrap: Reproducing Original \textBERT{}}
\label{sec:experiments}

We now discusses challenges in reproducing the performance of the original \textBERT{} checkpoint, using the Multi-Bootstrap procedure presented above.

The performance of the original \texttt{bert-base-uncased} checkpoint appears to be an outlier when viewed against the distribution of scores obtained using the \multiberts{} reproductions. 
Specifically, in reproducing the training recipe of \citet{devlin2018bert}, we found it difficult to simultaneously match performance on all tasks using a single set of hyperparameters. \citet{devlin2018bert} reports training for 1M steps. However, as shown in \autoref{fig:glue} and \ref{fig:squad}, models pretrained for 1M steps matched the original checkpoint on SQuAD but lagged behind on GLUE tasks; if pretraining continues to 2M steps, GLUE performance matches the original checkpoint but SQuAD performance is significantly higher. 

The above observations suggest two separate but related hypotheses (below) about the \textBERT{} pretraining procedure. In this section, we use the proposed Multi-Bootstrap procedure to test these hypotheses. 
\begin{enumerate}
    \item On most tasks, running \textBERT{} pretraining for 2M steps produces better models than 1M steps. We test this using paired Multi-Bootstrap (\S\ref{sec:1m2m}).
    \item The \multiberts{} training procedure outperforms the original \textBERT{} procedure on SQuAD. We test this using unpaired Multi-Bootstrap (\S\ref{sec:squad-repro}).
\end{enumerate}

\subsection{How many steps to pretrain?}
\label{sec:1m2m}

To test our first hypothesis, we use the proposed Multi-Bootstrap, letting $f$ be the predictor induced by the \textBERT{} pretraining procedure using the default 1M steps, and letting $f'$ be the predictor resulting from the proposed intervention of training to 2M steps. From a glance at the histograms in \autoref{fig:glue-sec5}, we can see that MNLI appears to be a case where 2M is generally better, while MRPC and RTE appear less conclusive. Multi-Bootstrap allows us to test this quantitatively using samples over both the seeds and the test examples. Results are shown in \autoref{tab:1m-vs-2m-boot}. We find that MNLI conclusively performs better ($\delta = 0.007$ with $p < 0.001$) with 2M steps; for RTE and MRPC we cannot reject the null hypothesis of no difference ($p=0.14$ and $p=0.56$ respectively). 

\begin{table}[ht!]
    \centering
    \begin{tabular}{@{}lrrr@{}}
    \toprule
    \textbf{}                              & \textbf{MNLI} & \textbf{RTE} & \textbf{MRPC} \\ \midrule
    \textbf{$\theta_{f}$} (1M steps)         & 0.837         & 0.644        & 0.861         \\
    \textbf{$\theta_{f'}$} (2M steps)        & 0.844         & 0.655        & 0.860         \\
    \textbf{$\delta = \theta_{f'} - \theta_f$}                  & 0.007         & 0.011        & -0.001        \\ \midrule
    \shortstack[l]{$p$-value \\ ($H_0$ that $\delta \le 0$)} & $<$ 0.001             & 0.141        & 0.564         \\ \bottomrule
    \end{tabular}
    \caption{Expected scores (accuracy), effect sizes, and $p$-values from Multi-Bootstrap on selected GLUE tasks. We pre-select the best fine-tuning learning rate by averaging over runs; this is 3e-5 for checkpoints at 1M steps, and 2e-5 for checkpoints at 2M pretraining steps. All tests use 1000 bootstrap samples, in paired mode on the five seeds for which both 1M and 2M steps are available.}
    \label{tab:1m-vs-2m-boot}
\end{table}

As an example of the utility of this procedure, \autoref{fig:mnli-mantaray} shows the distribution of individual samples of $L$ for the intervention $f'$ and baseline $f$ from this bootstrap procedure (which we denote as $L'$ and $L$, respectively). The distributions overlap significantly, but the samples are highly correlated due to the paired sampling, and we find that individual samples of the \emph{difference} $(L' - L)$ are nearly always positive.

\begin{figure}[ht!]
    \centering
    % \includegraphics[width=0.63\columnwidth]{figures/mnli_multibootstrap}
    % \includegraphics[width=0.35\columnwidth]{figures/mnli_deltas}
    \includegraphics[width=.5\textwidth]{figures/mnli_boot_mantas}
    \caption{Distribution of estimated performance on MNLI across boostrap samples, for runs with 1M or 2M steps. Individual samples of $L(S, (X,Y))$ and $L'(S, (X,Y))$ on the left, deltas $L'(S, (X, Y)) - L(S, (X,Y))$ shown on the right. Bootstrap experiment is run as in Table~\ref{tab:1m-vs-2m-boot}, which gives $\delta = 0.007$ with $p < 0.001$.}
    \label{fig:mnli-mantaray}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{figures/2m_vs_1m.png}
    % \vspace*{-8mm}
    \caption{Distribution of the performance on GLUE dev sets, showing only runs with the best selected learning rate for each task. Each plot shows 25 points (5 finetuning x 5 pretraining) for each of the 1M and 2M-step versions of each of the pretraining runs for which we release intermediate checkpoints (\S\ref{sec:release}).
    % The dashed line indicates the performance of the original \textBERT{} release.
    }
    \label{fig:glue-sec5}
\end{figure}


\subsection{Does the \multiberts{} procedure outperform original \textBERT{} on SQuAD?}
\label{sec:squad-repro}
To test our second hypothesis, i.e., that the \multiberts{} procedure outperforms original \textBERT{} on SQuAD, we must use the unpaired Multi-Bootstrap procedure. In particular, we are limited to the case in which we only have a point estimate of $L'(S)$, because we only have a single estimate of the performance of our baseline model $f'$ (the original \textBERT{} checkpoint). However, the Multi-Bootstrap procedure still allows us to estimate variance across our \multiberts{} seeds and across the examples in the evaluation set. On SQuAD 2.0, we find that the \multiberts{} models trained for 2M steps outperform original \textBERT{} with a 95\% confidence range of 1.9\% to 2.9\% and $p < 0.001$ for the null hypothesis, corroborating our intuition from \autoref{fig:squad}.

We include notebooks for the above analyses in our code release.
